Constraints-Informed Neural-Laguerre Approximation of Nonlinear MPC with Application in Power Electronics

This paper considers learning online (implicit) nonlinear model predictive control (MPC) laws using neural networks and Laguerre functions. Firstly, we parameterize the control sequence of nonlinear MPC using Laguerre functions, which typically yields a smoother control law compared to the original nonlinear MPC law. Secondly, we employ neural networks to learn the coefficients of the Laguerre nonlinear MPC solution, which comes with several benefits, namely the dimension of the learning space is dictated by the number of Laguerre functions and the complete predicted input sequence can be used to learn the coefficients. To mitigate constraints violation for neural approximations of nonlinear MPC, we develop a constraints-informed loss function that penalizes the violation of polytopic state constraints during learning. Box input constraints are handled by using a clamp function in the output layer of the neural network. We demonstrate the effectiveness of the developed framework on a nonlinear buck-boost converter model with sampling rates in the sub-millisecond range, where online nonlinear MPC would not be able to run in real time. The developed constraints-informed neural-Laguerre approximation yields similar performance with long-horizon online nonlinear MPC, but with execution times of a few microseconds, as validated on a field-programmable gate array (FPGA) platform.

==> Fig/NN.tex <==
\begin{tikzpicture}
    \fill[mlBlue!20,rounded corners] (-0.5, -2.3) rectangle (0.5, 0.8) {};
    \fill[mlBlue!40,rounded corners] (1.1-0.5, -2.3) rectangle (1.1+0.5, 0.8) {};
    \fill[mlBlue!60,rounded corners] (2.2-0.5, -2.3) rectangle (2.2+0.5, 0.8) {};
    \fill[mlBlue!80,rounded corners] (3.3-0.5, -2.3) rectangle (3.3+0.5, 0.8) {};

    \draw (0, 1.2) node[align=left, below, text=black] {\footnotesize Input};
    \draw (1.1, 1.2) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (2.2, 1.2) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (3.3, 1.2) node[align=left, below, text=black] {\footnotesize Output};

    % Input
    \node[] (x1) at (-1,0) {\footnotesize $x_{1,k}$};
    \node[] (x2) at (-1,-0.7) {\footnotesize $x_{2,k}$};
    \node[] at (-1,-1.05) {\scriptsize $\vdots$};
    \node[] (xn) at (-1,-1.6) {\footnotesize $x_{n,k}$};
    \node[circle,draw,very thick,minimum size=0.4cm] (i1) at (0,0) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (i2) at (0,-0.7) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (i3) at (0,-1.6) {};
    % Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h11) at (1.1,0.4) {};
    \draw let \p1=(h11.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h12) at (1.1,-0.3) {};
    \draw let \p1=(h12.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h13) at (1.1,-1) {};
    \draw let \p1=(h13.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h14) at (1.1,-1.9) {};
    \draw let \p1=(h14.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    % Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h21) at (2.2,0.4) {};
    \draw let \p1=(h21.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h22) at (2.2,-0.3) {};
    \draw let \p1=(h22.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h23) at (2.2,-1) {};
    \draw let \p1=(h23.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h24) at (2.2,-1.9) {};
    \draw let \p1=(h24.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    % Output layer
    \node[circle,draw,very thick,minimum size=0.4cm] (o1) at (3.3,-0.7) {};
    \draw let \p1=(o1.south) in [black, domain=-1:1,shift=(\p1),scale=0.1,yshift=14mm] plot ({\x},{1.5/(1+exp(-9*\x))});
    % u0 layer
    \node[] (u) at (4.4,-0.7) {\footnotesize$\hat{u}_{0|k}$};

    % Node-to-node lines
    \draw[-latex] ([xshift=-1mm] x1.east) -- (i1.west);
    \draw[-latex] ([xshift=-1mm] x2.east) -- (i2.west);
    \draw[-latex] ([xshift=-1mm] xn.east) -- (i3.west);
    \draw[-latex] (i1.east) -- (h11.west);
    \draw[-latex] (i1.east) -- (h12.west);
    \draw[-latex] (i1.east) -- (h13.west);
    \draw[-latex] (i1.east) -- (h14.west);
    \draw[-latex] (i2.east) -- (h11.west);
    \draw[-latex] (i2.east) -- (h12.west);
    \draw[-latex] (i2.east) -- (h13.west);
    \draw[-latex] (i2.east) -- (h14.west);
    \draw[-latex] (i3.east) -- (h11.west);
    \draw[-latex] (i3.east) -- (h12.west);
    \draw[-latex] (i3.east) -- (h13.west);
    \draw[-latex] (i3.east) -- (h14.west);

    \draw[-latex] (h11.east) -- (h21.west);
    \draw[-latex] (h11.east) -- (h22.west);
    \draw[-latex] (h11.east) -- (h23.west);
    \draw[-latex] (h11.east) -- (h24.west);
    \draw[-latex] (h12.east) -- (h21.west);
    \draw[-latex] (h12.east) -- (h22.west);
    \draw[-latex] (h12.east) -- (h23.west);
    \draw[-latex] (h12.east) -- (h24.west);
    \draw[-latex] (h13.east) -- (h21.west);
    \draw[-latex] (h13.east) -- (h22.west);
    \draw[-latex] (h13.east) -- (h23.west);
    \draw[-latex] (h13.east) -- (h24.west);
    \draw[-latex] (h14.east) -- (h21.west);
    \draw[-latex] (h14.east) -- (h22.west);
    \draw[-latex] (h14.east) -- (h23.west);
    \draw[-latex] (h14.east) -- (h24.west);

    \draw[-latex] (h21.east) -- (o1.west);
    \draw[-latex] (h22.east) -- (o1.west);
    \draw[-latex] (h23.east) -- (o1.west);
    \draw[-latex] (h24.east) -- (o1.west);

    \draw[-latex] (o1.east) -- ([xshift=0.7mm] u.west);

    % Dotted lines
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] i2.south) -- ([yshift=1mm] i3.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h13.south) -- ([yshift=1mm] h14.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h23.south) -- ([yshift=1mm] h24.north);
\end{tikzpicture}

==> Fig/NN_Lag.tex <==
% \begin{tikzpicture}
%             \fill[mlOrange!20,rounded corners] (-0.5, -2.3) rectangle (0.5, 0.8) {};
%             \fill[mlOrange!40,rounded corners] (1.1-0.5, -2.3) rectangle (1.1+0.5, 0.8) {};
%             \fill[mlOrange!60,rounded corners] (2.2-0.5, -2.3) rectangle (2.2+0.5, 0.8) {};
%             \fill[mlOrange!80,rounded corners] (3.3-0.5, -2.3) rectangle (3.3+0.5, 0.8) {};
            
%             \draw (0, 1.2) node[align=left, below, text=black] {\footnotesize Input};
%             \draw (1.1, 1.2) node[align=left, below, text=black] {\footnotesize Hidden};
%             \draw (2.2, 1.2) node[align=left, below, text=black] {\footnotesize Hidden};
%             \draw (3.6, 1.2) node[align=left, below, text=black] {\footnotesize Coefficients};
        
%             % Input
%             \node[] (x) at (-1,-0.7) {\footnotesize$\begin{bmatrix} x_{1,k}\\ x_{2,k}\\ \vdots \\ x_{n_x,k} \end{bmatrix}$};
%             \node[circle,draw,very thick,minimum size=0.4cm] (x1) at (0,0) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (x2) at (0,-0.7) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (x3) at (0,-1.6) {};
%             % Hidden layer
%             \node[circle,draw,very thick,minimum size=0.4cm] (h11) at (1.1,0.4) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (h12) at (1.1,-0.3) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (h13) at (1.1,-1) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (h14) at (1.1,-1.9) {};
%             % Hidden layer
%             \node[circle,draw,very thick,minimum size=0.4cm] (h21) at (2.2,0.4) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (h22) at (2.2,-0.3) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (h23) at (2.2,-1) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (h24) at (2.2,-1.9) {};  
%             % Coefficient layer
%             \node[circle,draw,very thick,minimum size=0.4cm] (o1) at (3.3,0) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (o2) at (3.3,-0.7) {};
%             \node[circle,draw,very thick,minimum size=0.4cm] (o3) at (3.3,-1.6) {};
%             \node[] (eta) at (4.35,-0.7) {\footnotesize $\begin{bmatrix} \hat{\eta}_{k,1}\\ \hat{\eta}_{k,2}\\ \vdots \\ \hat{\eta}_{k,M} \end{bmatrix}$};
%             % Laguerre layer
%             % \draw[rounded corners,very thick] (5.3-0.3, -0.7-0.3) rectangle (5.3+0.3, -0.7+0.3) {};
%             % \node[] (L) at (5.3, -0.7) {\footnotesize$L$};
%             % Output
%             % \node[] (U) at (6.3,-0.7) {\footnotesize$\begin{bmatrix} \hat{u}_{0|k}\\ \hat{u}_{1|k}\\ \vdots \\ \hat{u}_{N-1|k} \end{bmatrix}$};

%             % Node-to-node lines
%             \draw[-latex] ([xshift=-1mm] x.east) -- (i1.west);
%             \draw[-latex] ([xshift=-1mm] x.east) -- (i2.west);
%             \draw[-latex] ([xshift=-1mm] x.east) -- (i3.west);
%             \draw[-latex] (x1.east) -- (h11.west);
%             \draw[-latex] (x1.east) -- (h12.west);
%             \draw[-latex] (x1.east) -- (h13.west);
%             \draw[-latex] (x1.east) -- (h14.west);
%             \draw[-latex] (x2.east) -- (h11.west);
%             \draw[-latex] (x2.east) -- (h12.west);
%             \draw[-latex] (x2.east) -- (h13.west);
%             \draw[-latex] (x2.east) -- (h14.west);
%             \draw[-latex] (x3.east) -- (h11.west);
%             \draw[-latex] (x3.east) -- (h12.west);
%             \draw[-latex] (x3.east) -- (h13.west);
%             \draw[-latex] (x3.east) -- (h14.west);

%             \draw[-latex] (h11.east) -- (h21.west);
%             \draw[-latex] (h11.east) -- (h22.west);
%             \draw[-latex] (h11.east) -- (h23.west);
%             \draw[-latex] (h11.east) -- (h24.west);
%             \draw[-latex] (h12.east) -- (h21.west);
%             \draw[-latex] (h12.east) -- (h22.west);
%             \draw[-latex] (h12.east) -- (h23.west);
%             \draw[-latex] (h12.east) -- (h24.west);
%             \draw[-latex] (h13.east) -- (h21.west);
%             \draw[-latex] (h13.east) -- (h22.west);
%             \draw[-latex] (h13.east) -- (h23.west);
%             \draw[-latex] (h13.east) -- (h24.west);
%             \draw[-latex] (h14.east) -- (h21.west);
%             \draw[-latex] (h14.east) -- (h22.west);
%             \draw[-latex] (h14.east) -- (h23.west);
%             \draw[-latex] (h14.east) -- (h24.west);

%             \draw[-latex] (h21.east) -- (o1.west);
%             \draw[-latex] (h22.east) -- (o1.west);
%             \draw[-latex] (h23.east) -- (o1.west);
%             \draw[-latex] (h24.east) -- (o1.west);
%             \draw[-latex] (h21.east) -- (o2.west);
%             \draw[-latex] (h22.east) -- (o2.west);
%             \draw[-latex] (h23.east) -- (o2.west);
%             \draw[-latex] (h24.east) -- (o2.west);
%             \draw[-latex] (h21.east) -- (o3.west);
%             \draw[-latex] (h22.east) -- (o3.west);
%             \draw[-latex] (h23.east) -- (o3.west);
%             \draw[-latex] (h24.east) -- (o3.west);

%             \draw[-latex] (o1.east) -- ([xshift=2mm] eta.west);
%             \draw[-latex] (o2.east) -- ([xshift=2mm] eta.west);
%             \draw[-latex] (o3.east) -- ([xshift=2mm] eta.west);

%             \draw[-latex] ([xshift=-2mm] eta.east) -- ([xshift=-1mm] L.west);

%             \draw[-latex] ([xshift=1mm] L.east) -- ([xshift=2mm] U.west);

%             % Dotted lines
%             \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] i2.south) -- ([yshift=1mm] i3.north);
%             \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h13.south) -- ([yshift=1mm] h14.north);
%             \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h23.south) -- ([yshift=1mm] h24.north);
%             \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] o2.south) -- ([yshift=1mm] o3.north);
%         \end{tikzpicture}

\begin{tikzpicture}
    \fill[mlOrange!20,rounded corners] (-0.5, -2.3) rectangle (0.5, 0.8) {};
    \fill[mlOrange!40,rounded corners] (1.1-0.5, -2.3) rectangle (1.1+0.5, 0.8) {};
    \fill[mlOrange!60,rounded corners] (2.2-0.5, -2.3) rectangle (2.2+0.5, 0.8) {};
    \fill[mlOrange!80,rounded corners] (3.3-0.5, -2.3) rectangle (3.3+0.5, 0.8) {};
    \fill[black!25,rounded corners] (5.3-0.5, -2.3) rectangle (5.3+0.5, 0.8) {};
    
    \draw (0, 1.3) node[align=left, below, text=black] {\footnotesize Input};
    \draw (1.1, 1.3) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (2.2, 1.3) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (3.5, 1.3) node[align=left, below, text=black] {\footnotesize Coefficients};
    \draw (5.3, 1.3) node[align=left, below, text=black] {\footnotesize Laguerre};

    % Input
    \node[] (x1) at (-1,0) {\scriptsize $x_{1,k}$};
    \node[] (x2) at (-1,-0.7) {\scriptsize $x_{2,k}$};
    \node[] at (-1,-1.05) {\scriptsize $\vdots$};
    \node[] (xn) at (-1,-1.6) {\scriptsize $x_{n,k}$};
    \node[circle,draw,very thick,minimum size=0.4cm] (i1) at (0,0) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (i2) at (0,-0.7) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (i3) at (0,-1.6) {};
    % Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h11) at (1.1,0.4) {};
    \draw let \p1=(h11.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h12) at (1.1,-0.3) {};
    \draw let \p1=(h12.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h13) at (1.1,-1) {};
    \draw let \p1=(h13.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h14) at (1.1,-1.9) {};
    \draw let \p1=(h14.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    % Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h21) at (2.2,0.4) {};
    \draw let \p1=(h21.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h22) at (2.2,-0.3) {};
    \draw let \p1=(h22.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h23) at (2.2,-1) {};
    \draw let \p1=(h23.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h24) at (2.2,-1.9) {};
    \draw let \p1=(h24.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    % Coefficient layer
    \node[circle,draw,very thick,minimum size=0.4cm] (o1) at (3.3,0) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (o2) at (3.3,-0.7) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (o3) at (3.3,-1.6) {};
    \node[] (eta) at (3.3,0.5) {\scriptsize $\hat{\eta}_{k}$};
    % Laguerre layer
    \node[circle,draw,very thick,minimum size=0.4cm] (l1) at (5.3,0) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (l2) at (5.3,-0.7) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (l3) at (5.3,-1.6) {};
    \draw let \p1=(l1.south) in [black, domain=-1:1,shift=(\p1),scale=0.1,yshift=14mm] plot ({\x},{1.5/(1+exp(-9*\x))});
    \draw let \p2=(l2.south) in [black, domain=-1:1,shift=(\p2),scale=0.1,yshift=14mm] plot ({\x},{1.5/(1+exp(-9*\x))});
    \draw let \p3=(l3.south) in [black, domain=-1:1,shift=(\p3),scale=0.1,yshift=14mm] plot ({\x},{1.5/(1+exp(-9*\x))});        
    % Output
    \node[] (u0) at (6.4,0) {\scriptsize$\hat{u}_{0|k}$};
    \node[] (u1) at (6.4,-0.7) {\scriptsize$\hat{u}_{1|k}$};
    \node[] at (6.4,-1.05) {\scriptsize $\vdots$};
    \node[] (uNmin1) at (6.53,-1.6) {\scriptsize$\hat{u}_{N-1|k}$};

    % Node-to-node lines
    \draw[-latex] ([xshift=-1mm] x1.east) -- (i1.west);
    \draw[-latex] ([xshift=-1mm] x2.east) -- (i2.west);
    \draw[-latex] ([xshift=-1mm] xn.east) -- (i3.west);
    \draw[-latex] (i1.east) -- (h11.west);
    \draw[-latex] (i1.east) -- (h12.west);
    \draw[-latex] (i1.east) -- (h13.west);
    \draw[-latex] (i1.east) -- (h14.west);
    \draw[-latex] (i2.east) -- (h11.west);
    \draw[-latex] (i2.east) -- (h12.west);
    \draw[-latex] (i2.east) -- (h13.west);
    \draw[-latex] (i2.east) -- (h14.west);
    \draw[-latex] (i3.east) -- (h11.west);
    \draw[-latex] (i3.east) -- (h12.west);
    \draw[-latex] (i3.east) -- (h13.west);
    \draw[-latex] (i3.east) -- (h14.west);

    \draw[-latex] (h11.east) -- (h21.west);
    \draw[-latex] (h11.east) -- (h22.west);
    \draw[-latex] (h11.east) -- (h23.west);
    \draw[-latex] (h11.east) -- (h24.west);
    \draw[-latex] (h12.east) -- (h21.west);
    \draw[-latex] (h12.east) -- (h22.west);
    \draw[-latex] (h12.east) -- (h23.west);
    \draw[-latex] (h12.east) -- (h24.west);
    \draw[-latex] (h13.east) -- (h21.west);
    \draw[-latex] (h13.east) -- (h22.west);
    \draw[-latex] (h13.east) -- (h23.west);
    \draw[-latex] (h13.east) -- (h24.west);
    \draw[-latex] (h14.east) -- (h21.west);
    \draw[-latex] (h14.east) -- (h22.west);
    \draw[-latex] (h14.east) -- (h23.west);
    \draw[-latex] (h14.east) -- (h24.west);

    \draw[-latex] (h21.east) -- (o1.west);
    \draw[-latex] (h22.east) -- (o1.west);
    \draw[-latex] (h23.east) -- (o1.west);
    \draw[-latex] (h24.east) -- (o1.west);
    \draw[-latex] (h21.east) -- (o2.west);
    \draw[-latex] (h22.east) -- (o2.west);
    \draw[-latex] (h23.east) -- (o2.west);
    \draw[-latex] (h24.east) -- (o2.west);
    \draw[-latex] (h21.east) -- (o3.west);
    \draw[-latex] (h22.east) -- (o3.west);
    \draw[-latex] (h23.east) -- (o3.west);
    \draw[-latex] (h24.east) -- (o3.west);

    \draw[-latex] (o1.east) -- (l1.west);
    \draw[-latex] (o1.east) -- (l2.west);
    \draw[-latex] (o1.east) -- (l3.west);
    \draw[-latex] (o2.east) -- (l1.west);
    \draw[-latex] (o2.east) -- (l2.west);
    \draw[-latex] (o2.east) -- (l3.west);
    \draw[-latex] (o3.east) -- (l1.west);
    \draw[-latex] (o3.east) -- (l2.west);
    \draw[-latex] (o3.east) -- (l3.west);

    \draw[-latex] (l1.east) -- ([xshift=0.5mm] u0.west);
    \draw[-latex] (l2.east) -- ([xshift=0.5mm] u1.west);
    \draw[-latex] (l3.east) -- ([xshift=0.5mm] uNmin1.west);
    % Dotted lines
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] i2.south) -- ([yshift=1mm] i3.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h13.south) -- ([yshift=1mm] h14.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h23.south) -- ([yshift=1mm] h24.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] o2.south) -- ([yshift=1mm] o3.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] l2.south) -- ([yshift=1mm] l3.north);
\end{tikzpicture}

==> Fig/NN_Lag_V2.tex <==
\begin{tikzpicture}
    \fill[mlOrange!20,rounded corners] (-0.5, -2.3) rectangle (0.5, 0.8) {};
    \fill[mlOrange!40,rounded corners] (1.1-0.5, -2.3) rectangle (1.1+0.5, 0.8) {};
    \fill[mlOrange!60,rounded corners] (2.2-0.5, -2.3) rectangle (2.2+0.5, 0.8) {};
    \fill[mlOrange!80,rounded corners] (3.3-0.5, -2.3) rectangle (3.3+0.5, 0.8) {};
    \fill[black!25,rounded corners] (4.8-0.5, -2.3) rectangle (4.8+0.5, 0.8) {};
    
    \draw (0, -2.3) node[align=left, below, text=black] {\footnotesize Input};
    \draw (1.1, -2.3) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (2.2, -2.3) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (3.5, -2.3) node[align=left, below, text=black] {\footnotesize Coefficients};
    \draw (4.8, -2.3) node[align=left, below, text=black] {\footnotesize Laguerre};

    %% Input
    \node[] (x1) at (-1,-0.7) {\scriptsize $x_{k}$};
    \node[circle,draw,very thick,minimum size=0.4cm] (i1) at (0,-0.7) {};
    %% Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h11) at (1.1,0.4) {};
    \draw let \p1=(h11.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h12) at (1.1,-0.3) {};
    \draw let \p1=(h12.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h13) at (1.1,-1) {};
    \draw let \p1=(h13.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h14) at (1.1,-1.9) {};
    \draw let \p1=(h14.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    %% Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h21) at (2.2,0.4) {};
    \draw let \p1=(h21.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h22) at (2.2,-0.3) {};
    \draw let \p1=(h22.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h23) at (2.2,-1) {};
    \draw let \p1=(h23.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h24) at (2.2,-1.9) {};
    \draw let \p1=(h24.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    %% Coefficient layer
    \node[circle,draw,very thick,minimum size=0.4cm] (o1) at (3.3,0) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (o2) at (3.3,-0.7) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (o3) at (3.3,-1.6) {};
    \node[] (eta) at (3.3,0.5) {\scriptsize $\hat{\eta}_{k}$};
    %% Laguerre layer
    \node[circle,draw,very thick,minimum size=0.4cm] (l1) at (4.8,0) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (l2) at (4.8,-0.7) {};
    \node[circle,draw,very thick,minimum size=0.4cm] (l3) at (4.8,-1.6) {};
    \draw let \p1=(l1.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=18mm] plot ({\x},{2*min(0.25,max(-0.25,\x))});
    \draw let \p2=(l2.south) in [black, domain=-1:1,shift=(\p2),scale=0.12,yshift=18mm] plot ({\x},{2*min(0.25,max(-0.25,\x))});
    \draw let \p3=(l3.south) in [black, domain=-1:1,shift=(\p3),scale=0.12,yshift=18mm] plot ({\x},{2*min(0.25,max(-0.25,\x))});
    %% Output
    \node[] (u0) at (6.05,0) {\scriptsize$\hat{u}_{0|k}$};
    \node[] (u1) at (6.05,-0.7) {\scriptsize$\hat{u}_{1|k}$};
    \node[] at (6.1,-1.05) {\scriptsize $\vdots$};
    \node[] (uNmin1) at (6.17,-1.6) {\scriptsize$\hat{u}_{N-1|k}$};
    %% Constraint info
    \fill[black!75,rounded corners] (5.7, 0.6) rectangle (6.7, 1.2) {};
    \node[] (f) at (6.2,0.9) {\scriptsize\textcolor{white}{$f(x,\hat{u})$}};
    \node[] (xPlus) at (7.2,0.95) {\scriptsize$x^+$};
    \draw[-latex,tips=true] (-0.7,-0.7) -- ++(0,1.7) -- ([xshift=-0.5mm, yshift=1mm] f.west);
    \draw[-latex,tips=true] (5.45,0) -- ++(0,0.8) -- ([xshift=-0.5mm, yshift=-1mm] f.west);
    \draw[-latex] ([xshift=0.5mm] f.east) -- ([xshift=0.5mm, yshift=-0.5mm] xPlus.west);
    
    %% Node-to-node lines
    \draw[-latex] ([xshift=-1mm] x1.east) -- (i1.west);
    \draw[-latex] (i1.east) -- (h11.west);
    \draw[-latex] (i1.east) -- (h12.west);
    \draw[-latex] (i1.east) -- (h13.west);
    \draw[-latex] (i1.east) -- (h14.west);

    \draw[-latex] (h11.east) -- (h21.west);
    \draw[-latex] (h11.east) -- (h22.west);
    \draw[-latex] (h11.east) -- (h23.west);
    \draw[-latex] (h11.east) -- (h24.west);
    \draw[-latex] (h12.east) -- (h21.west);
    \draw[-latex] (h12.east) -- (h22.west);
    \draw[-latex] (h12.east) -- (h23.west);
    \draw[-latex] (h12.east) -- (h24.west);
    \draw[-latex] (h13.east) -- (h21.west);
    \draw[-latex] (h13.east) -- (h22.west);
    \draw[-latex] (h13.east) -- (h23.west);
    \draw[-latex] (h13.east) -- (h24.west);
    \draw[-latex] (h14.east) -- (h21.west);
    \draw[-latex] (h14.east) -- (h22.west);
    \draw[-latex] (h14.east) -- (h23.west);
    \draw[-latex] (h14.east) -- (h24.west);

    \draw[-latex] (h21.east) -- (o1.west);
    \draw[-latex] (h22.east) -- (o1.west);
    \draw[-latex] (h23.east) -- (o1.west);
    \draw[-latex] (h24.east) -- (o1.west);
    \draw[-latex] (h21.east) -- (o2.west);
    \draw[-latex] (h22.east) -- (o2.west);
    \draw[-latex] (h23.east) -- (o2.west);
    \draw[-latex] (h24.east) -- (o2.west);
    \draw[-latex] (h21.east) -- (o3.west);
    \draw[-latex] (h22.east) -- (o3.west);
    \draw[-latex] (h23.east) -- (o3.west);
    \draw[-latex] (h24.east) -- (o3.west);

    \draw[-latex] (o1.east) -- (l1.west);
    \draw[-latex] (o1.east) -- (l2.west);
    \draw[-latex] (o1.east) -- (l3.west);
    \draw[-latex] (o2.east) -- (l1.west);
    \draw[-latex] (o2.east) -- (l2.west);
    \draw[-latex] (o2.east) -- (l3.west);
    \draw[-latex] (o3.east) -- (l1.west);
    \draw[-latex] (o3.east) -- (l2.west);
    \draw[-latex] (o3.east) -- (l3.west);

    \draw[-latex] (l1.east) -- ([xshift=0.5mm] u0.west);
    \draw[-latex] (l2.east) -- ([xshift=0.5mm] u1.west);
    \draw[-latex] (l3.east) -- ([xshift=0.5mm] uNmin1.west);
    %% Dotted lines
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h13.south) -- ([yshift=1mm] h14.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h23.south) -- ([yshift=1mm] h24.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] o2.south) -- ([yshift=1mm] o3.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] l2.south) -- ([yshift=1mm] l3.north);
\end{tikzpicture}

==> Fig/NN_V2.tex <==
\begin{tikzpicture}
    \fill[mlBlue!20,rounded corners] (-0.5, -2.3) rectangle (0.5, 0.8) {};
    \fill[mlBlue!40,rounded corners] (1.1-0.5, -2.3) rectangle (1.1+0.5, 0.8) {};
    \fill[mlBlue!60,rounded corners] (2.2-0.5, -2.3) rectangle (2.2+0.5, 0.8) {};
    \fill[mlBlue!80,rounded corners] (3.3-0.5, -2.3) rectangle (3.3+0.5, 0.8) {};

    \draw (0, -2.3) node[align=left, below, text=black] {\footnotesize Input};
    \draw (1.1, -2.3) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (2.2, -2.3) node[align=left, below, text=black] {\footnotesize Hidden};
    \draw (3.3, -2.3) node[align=left, below, text=black] {\footnotesize Output};

    % Input
    \node[] (x1) at (-1,-0.7) {\footnotesize $x_{k}$};
    \node[circle,draw,very thick,minimum size=0.4cm] (i1) at (0,-0.7) {};
    % Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h11) at (1.1,0.4) {};
    \draw let \p1=(h11.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h12) at (1.1,-0.3) {};
    \draw let \p1=(h12.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h13) at (1.1,-1) {};
    \draw let \p1=(h13.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h14) at (1.1,-1.9) {};
    \draw let \p1=(h14.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    % Hidden layer
    \node[circle,draw,very thick,minimum size=0.4cm] (h21) at (2.2,0.4) {};
    \draw let \p1=(h21.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h22) at (2.2,-0.3) {};
    \draw let \p1=(h22.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h23) at (2.2,-1) {};
    \draw let \p1=(h23.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    \node[circle,draw,very thick,minimum size=0.4cm] (h24) at (2.2,-1.9) {};
    \draw let \p1=(h24.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=13mm] plot ({\x},{max(0,\x)});
    % Output layer
    \node[circle,draw,very thick,minimum size=0.4cm] (o1) at (3.3,-0.7) {};
    \draw let \p1=(o1.south) in [black, domain=-1:1,shift=(\p1),scale=0.12,yshift=18mm] plot ({\x},{2*min(0.25,max(-0.25,\x))});
    % u0 layer
    \node[] (u) at (4.7,-0.7) {\footnotesize$\hat{u}_{0|k}$};
    %% Constraint info
    \fill[black!75,rounded corners] (4.5, 0.6) rectangle (5.5, 1.2) {};
    \node[] (f) at (5,0.9) {\scriptsize\textcolor{white}{$f(x,\hat{u})$}};
    \node[] (xPlus) at (6.1,0.95) {\scriptsize$x^+$};
    \draw[-latex,tips=true] (-0.7,-0.7) -- ++(0,1.7) -- ([xshift=-0.5mm, yshift=1mm] f.west);
    \draw[-latex,tips=true] (4,-0.7) -- ++(0,1.5) -- ([xshift=-0.5mm, yshift=-1mm] f.west);
    \draw[-latex] ([xshift=0.5mm] f.east) -- ([xshift=0.5mm, yshift=-0.5mm] xPlus.west);

    % Node-to-node lines
    \draw[-latex] ([xshift=-1mm] x1.east) -- (i1.west);
    \draw[-latex] (i1.east) -- (h11.west);
    \draw[-latex] (i1.east) -- (h12.west);
    \draw[-latex] (i1.east) -- (h13.west);
    \draw[-latex] (i1.east) -- (h14.west);

    \draw[-latex] (h11.east) -- (h21.west);
    \draw[-latex] (h11.east) -- (h22.west);
    \draw[-latex] (h11.east) -- (h23.west);
    \draw[-latex] (h11.east) -- (h24.west);
    \draw[-latex] (h12.east) -- (h21.west);
    \draw[-latex] (h12.east) -- (h22.west);
    \draw[-latex] (h12.east) -- (h23.west);
    \draw[-latex] (h12.east) -- (h24.west);
    \draw[-latex] (h13.east) -- (h21.west);
    \draw[-latex] (h13.east) -- (h22.west);
    \draw[-latex] (h13.east) -- (h23.west);
    \draw[-latex] (h13.east) -- (h24.west);
    \draw[-latex] (h14.east) -- (h21.west);
    \draw[-latex] (h14.east) -- (h22.west);
    \draw[-latex] (h14.east) -- (h23.west);
    \draw[-latex] (h14.east) -- (h24.west);

    \draw[-latex] (h21.east) -- (o1.west);
    \draw[-latex] (h22.east) -- (o1.west);
    \draw[-latex] (h23.east) -- (o1.west);
    \draw[-latex] (h24.east) -- (o1.west);

    \draw[-latex] (o1.east) -- ([xshift=0.7mm] u.west);

    % Dotted lines
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h13.south) -- ([yshift=1mm] h14.north);
    \draw[decorate sep={0.4mm}{1.2mm},fill] ([yshift=-1mm] h23.south) -- ([yshift=1mm] h24.north);
\end{tikzpicture}
